High-Performance Trajectory Tracking MPC for Quadcopters with Coupled Time-Varying Constraints and Stability Proofs

In this paper, we present a cascade control structure to address the trajectory tracking problem for quadcopters, ensuring uniform global asymptotic stability of the state tracking error dynamics. An MPC strategy based on a 12-dimensional prediction model is proposed for the outer loop, explicitly accounting for time-varying coupled constraints, where multiple variables are interdependent and need to be handled together. The outer-loop controller generates an acceleration reference, which is then converted into attitude and angular velocity references, later tracked by a nonlinear inner-loop controller. Numerical simulations validate the approach, demonstrating enhanced performance in precise and fast tracking by imposing less conservative constraints than existing approaches, while still guaranteeing stability.

==> Section3/problem-statement.tex <==
%In this section, we review the verification problem and the assumptions that we consider to solve this problem.

